ACDG-VTON: Accurate and Contained Diffusion Generation for Virtual Try-On

Virtual Try-on (VTON) involves generating images of a person wearing selected garments. Diffusion-based methods, in particular, can create high-quality images, but they struggle to maintain the identities of the input garments. We identified this problem stems from the specifics in the training formulation for diffusion. To address this, we propose a unique training scheme that limits the scope in which diffusion is trained. We use a control image that perfectly aligns with the target image during training. In turn, this accurately preserves garment details during inference. We demonstrate our method not only effectively conserves garment details but also allows for layering, styling, and shoe try-on. Our method runs multi-garment try-on in a single inference cycle and can support high-quality zoomed-in generations without training in higher resolutions. Finally, we show our method surpasses prior methods in accuracy and quality.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}
% Generative AI has demonstrated astonishing capabilities in producing high-quality, lifelike images. These methodologies have paved the way for innovative applications, including the creation of new art, style transfer between pictures, and generating high-resolution images from text. However, despite the amazing results of methods like Stable Diffusion \cite{rombach2021highresolution}, many real-life applications necessitate image adherence to very specific specifications.

Virtual Try-on (VTON) is hard for modern generative models because VTON methods, to be commercially successful, must actually show a {\em specific} garment {\em accurately}. Achieving this criterion is a demanding task (Fig.~\ref{fig:teaser} and~\ref{fig:sota_comparison}). Together with accuracy, VTON pipelines must also offer quality and controllability to be commercially appealing. At present, GANs combined with warping techniques are the most accurate and controllable methods, but they often suffer from quality issues. Conversely, diffusion methods provide high quality, but it is difficult to contain a diffusion method to prevent it from inventing non-existent details. Even diffusion approaches that integrate warping steps tend to lose garment details. We introduce a novel warp-then-diffuse method that is accurate to the garment details, notably improves image quality, and allows for garment controllability. During inference, our approach utilizes garment warps to create a control image that is fed in as a reference for the diffusion denoiser. During training, however, we craft a control image that is aligned with the target image. This alignment results in accurate garment details at inference time and facilitates the ability to generate high-resolution close-ups for VTON. 
% obtained by training at different scales. 
%Our results, both qualitative and quantitative, demonstrate that garment features like text, logos, textures, and patterns are better preserved compared to other diffusion-based methods.
Qualitative results show garment features (text, logos, textures, and patterns) are better preserved compared to other diffusion-based methods.  Our method outperforms all others in standard quantitative metrics. Quantitative user studies show a pronounced preference for our method in accuracy. Finally, quantitative user studies show a significant gain in quality results from applying properly contained diffusion as a generator. 
%Careful alignment between the initialization and the desired image results in accurate garment details. 
%Estimates at more than one scale are used to  insight that the initialization is incredibly important for diffusion-based models and develop a method to use warps to provide us with a good approximate initialization. More importantly, we create a training strategy that accurately retains details from the clothing warps.  Finally, because our method accurately preserves warp details, it enables us to resolve the problem of detail loss in high-frequency areas when using VAEs. Our strategy allows us to focus on those high-frequency image regions and preserve the details, and allows us to do novel tasks such as generating high-resolution zoomed regions of regions on the model for virtual try-on.

% One task of generative AI is virtual try-on (VTON), which aims to create images of a select person wearing chosen garments. 
%While many successful attempts have generated realistic images of people wearing clothes, getting the fine details correct still presents a significant challenge. The initial methods of virtual try-on have a range of problems, such as functioning with only upper garments, lack of support for layering, inferior quality images, and inaccurate representation of garments. 
% More recent works improve on these problems, but still lack realism and have poor image quality. Moreover, newer diffusion-based techniques improve the image quality but show slip-ups in preserving garment identities.
% We want to build a VTON pipeline that can satisfy several criteria: \textbf{accuracy, quality, controllability}.

\begin{figure}[tb]
  \centering
    \includegraphics[width=1.0\textwidth]{images/teaser.jpg}
  \caption{Accuracy refers to how well the generated items generate the details of the actual garments. Our method preserves garment details such as graphics, text, and patterns better than diffusion-based try-on methods. LaDI-VTON~\cite{Morelli2023LadiVTON} and StableVITON~\cite{Kim2023StableVITON} are not accurate because both methods alter and hallucinate details on the garment. Furthermore, our proposed zoom-in method can make additional improvements to preserve the details that VAEs may distort (e.g. text).}
  \label{fig:teaser}
\end{figure}

% \subsection{What Should VTON Do?}
VTON methods must be evaluated qualitatively, and the criterion used matters. We see three major axes of evaluation: accuracy, quality and contollability. We describe each explicitly to avoid ambiguities or confusion.

\begin{figure}[tb]
  \centering
    \includegraphics[width=0.98\textwidth]{images/vae_encode_decode.jpg}
  \caption{VAEs~\cite{Kingma2014} can cause loss of high-frequency details. If we take a 512x512 crop from a larger image and encode and decode the image through a VAE, certain details will be altered because the VAE dictionary cannot reconstruct high-frequency features. The button's colors are changed, the angel's face and body are altered, and the pattern near the hem differs (see red arrows). We can work around this issue by upsampling the 512x512 crop to 1024x1024. The details are better preserved if we encode and decode the 1024x1024 image through VAE (see green arrows). 
  % This means our full body image must be at 2048x2048 resolution
  }
  \label{fig:vae_encode_decode}
\end{figure}

\textbf{Accuracy} refers to how well the generated items mirror the characteristics of the actual garments. We can measure accuracy by how effectively a garment's colors, shapes, textures, logos, proportions, and other defining aspects are retained. This is fundamental to the VTON task because we are not aiming to generate any garment, but a specific garment. Missing details or misrepresented attributes could alter the garment's identity. For example, if a maxi skirt is rendered shorter, it becomes a midi skirt. Similarly, changing a garment's texture or material may reclassify it in a store's inventory.  As a result, we believe accuracy is the most important characteristic of virtual try-on.  % and other criteria follow after accuracy.

Diffusion-based methods~\cite{Morelli2023LadiVTON, Kim2023StableVITON, Gou2023DCIVTON, Xie2023GPVTON} face accuracy issues due to two reasons: 1) diffusion methods tend to hallucinate details, and 2) most diffusion methods use a Variational Autoencoder (VAE)~\cite{Kingma2014} for efficiency, which can remove high-frequency details. Notice in Fig.~\ref{fig:teaser}, diffusion methods like LaDI-VTON~\cite{Morelli2023LadiVTON} and StableVITON~\cite{Kim2023StableVITON} create designs that were not included in the input garment. Additionally, in Fig.~\ref{fig:vae_encode_decode}, we reveal that VAEs may distort image details because the size of the VAE dictionary is limited, and it modifies high-frequency details. This distortion can be reduced by training in higher resolutions, but this solution may not always be computationally feasible.

\textbf{Quality} refers to the generated images' realism and visual appeal. In its simplest form, a virtual try-on system could be implemented as a collage by cutting out a face and roughly superimposing various garments on a body template. While this would provide a basic vision of how the clothes could appear, it would lack intricate details such as how the garments drape, their interactions with other clothing, or how shadows might appear on a real person. The lifelike representation of showcasing the garments is important in an industry where product perception is everything to lure buyers and draw attention. 

\textbf{Garment Controllability} refers to how much we can influence the generated output and the ability to layer garments and control different styling options. Layering garments refers to the order in which clothes are donned, while styling options reflect how each piece is worn - for instance, whether outerwear is open or closed, tops are tucked or not, and clothes are worn loosely or tightly. The way people wear clothes varies greatly, and users must have control over how they style the garments for a realistic try-on experience.
% Both garment layering and styling involve the ability to change a particular garment without affecting the appearance of other garments not involved in that change.
% In Fig.~\ref{fig:controllability}, we compare Rendering Policies and Outfit Anyone to illustrate garment controllability. Notice Rendering Policies is able to layer garments, control how garments are worn (closed/open outerwear and tucked/untucked tops), and garments not adjusted don't change between generations. In contrast, TryOnDiffusion cannot consistently control the generation of the garment and outfits are worn differently in every generation.

Our work employs Stable Diffusion~\cite{rombach2021highresolution} to produce warp-based VTON generations that meet all three criteria and have several key contributions. 
% We leverage the insight that the initialization is incredibly important for diffusion-based models and develop a method to use warps to provide us with a good approximate initialization. More importantly, 
First, we devise a VTON training strategy that effectively retains the details from warped garments. We demonstrate that our method preserves garment features like text, logos, textures, and patterns more effectively than other GAN-based and diffusion-based methods. Second, we present a novel capability to generate zoomed-in regions for virtual try-on to counteract the loss of high-frequency details when using VAEs~\cite{Kingma2014} without needing to train in higher resolution. Lastly, our method allows for the simultaneous generation of multiple garments in a single diffusion inference cycle while offering control over sizing and style.

